TOCTOU Resilient Attestation for IoT Networks (Full Version)

Internet-of-Things (IoT) devices are increasingly common in both consumer and industrial settings, often performing safety-critical functions. Although securing these devices is vital, manufacturers typically neglect security issues or address them as an afterthought. This is of particular importance in IoT networks, e.g., in the industrial automation settings. To this end, network attestation -- verifying the software state of all devices in a network -- is a promising mitigation approach. However, current network attestation schemes have certain shortcomings: (1) lengthy TOCTOU (Time-Of-Check-Time-Of-Use) vulnerability windows, (2) high latency and resource overhead, and (3) susceptibility to interference from compromised devices. To address these limitations, we construct TRAIN (TOCTOU-Resilient Attestation for IoT Networks), an efficient technique that minimizes TOCTOU windows, ensures constant-time per-device attestation, and maintains resilience even with multiple compromised devices. We demonstrate TRAIN's viability and evaluate its performance via a fully functional and publicly available prototype.

==> content/11-ethics.tex <==
\newpage

\section* {\centering  Data Availability}

The implementation of \system is open-sourced. It is 
currently available at \cite{TRAPSAnonOpenSource}, with detailed 
instructions on how to reproduce \system and its evaluation. 
If/when this paper is accepted, we will make it publicly 
available.\\ \\

